Approximating Cross-validatory Predictive Evaluation in Bayesian Latent Variables Models with Integrated IS and WAIC

A natural method for approximating out-of-sample predictive evaluation is leave-one-out cross-validation (LOOCV) --- we alternately hold out each case from a full data set and then train a Bayesian model using Markov chain Monte Carlo (MCMC) without the held-out; at last we evaluate the posterior predictive distribution of all cases with their actual observations. However, actual LOOCV is time-consuming. This paper introduces two methods, namely iIS and iWAIC, for approximating LOOCV with only Markov chain samples simulated from a posterior based on a \textit{full} data set. iIS and iWAIC aim at improving the approximations given by importance sampling (IS) and WAIC in Bayesian models with possibly correlated latent variables. In iIS and iWAIC, we first integrate the predictive density over the distribution of the latent variables associated with the held-out without reference to its observation, then apply IS and WAIC approximations to the integrated predictive density. We compare iIS and iWAIC with other approximation methods in three real data examples that respectively use mixture models, models with correlated spatial effects, and a random effect logistic model. Our empirical results show that iIS and iWAIC give substantially better approximates than non-integrated IS and WAIC and other methods.

==> msel_count.tex <==
% latex table generated in R 3.1.0 by xtable 1.7-3 package
% Sun Dec  7 15:41:43 2014
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrr}
  \hline
$K$ & IS & WAIC & iIS & iWAIC & DIC \\ 
  \hline
2 & 0 & 0 & 0 & 0 & 2 \\ 
  3 & 0 & 0 & 15 & 15 & 94 \\ 
  4 & 6 & 15 & 39 & 37 & 4 \\ 
  5 & 10 & 4 & 21 & 20 & 0 \\ 
  6 & 30 & 8 & 11 & 13 & 0 \\ 
  7 & 54 & 73 & 14 & 15 & 0 \\ 
   \hline
\end{tabular}
\end{table}


==> sim-icmean.tex <==
% latex table generated in R 3.1.0 by xtable 1.7-3 package
% Sun Dec  7 15:41:43 2014
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrr}
  \hline
 & IS & WAIC & iIS & iWAIC & DIC \\ 
  \hline
 2 & 1112.48 & 1103.95 & 1181.60 & 1182.33 & 1248.97 \\ 
  3 & 922.88 & 751.58 & 1105.18 & 1105.11 & 990.51 \\ 
  4 & 827.06 & 682.62 & 1099.42 & 1099.26 & 1572.80 \\ 
  5 & 810.42 & 674.39 & 1099.18 & 1098.96 & 1562.05 \\ 
  6 & 801.24 & 669.57 & 1099.60 & 1099.31 & 1630.02 \\ 
  7 & 796.65 & 666.39 & 1100.09 & 1099.77 & 1700.12 \\ 
   \hline
\end{tabular}
\end{table}

